Optimal Functional Bilinear Regression with Two-way Functional Covariates via Reproducing Kernel Hilbert Space

Traditional functional linear regression usually takes a one-dimensional functional predictor as input and estimates the continuous coefficient function. Modern applications often generate two-dimensional covariates, which become matrices when observed at grid points. To avoid the inefficiency of the classical method involving estimation of a two-dimensional coefficient function, we propose a functional bilinear regression model, and introduce an innovative three-term penalty to impose roughness penalty in the estimation. The proposed estimator exhibits minimax optimal property for prediction under the framework of reproducing kernel Hilbert space. An iterative generalized cross-validation approach is developed to choose tuning parameters, which significantly improves the computational efficiency over the traditional cross-validation approach. The statistical and computational advantages of the proposed method over existing methods are further demonstrated via simulated experiments, the Canadian weather data, and a biochemical long-range infrared light detection and ranging data.

==> TEX/KEEP_old_theory_with_diagonalization_KEEP.tex <==
\section{Theoretical results: optimal rate of convergence}
\label{sec:theory}

\subsection{Preliminary}
\label{ssec:theory-preliminary}

In this section, we introduce some more notations and assumptions on the reproducing kernels and covariance functions that will be used in the development of the minimax rate of convergence.

From the methodology point of view, it is implicitly assumed that the two domains, the covariance structures of the two dimensions, and the levels of smoothness of the two coefficient functions may be different and require different penalties thereby. For notational simplicity, throughout the theoretical section, we assume that they are the same, that is, $\T_1 = \T_2 = \T, ~K_1=K_2=K, ~C_\alpha=C_\beta=C$ and $\lambda_\alpha=\lambda_\beta=\lambda$. 
%But the discussions and theorems in this section are still applicable with slight adjustment when the two domains and their corresponding properties are different.
It follows that the $\zerosnorm{\cdot}$ and $\zerotnorm{\cdot}$ norms are identical, and hence we write them as $\zeronorm{\cdot}$. The theoretical results and proofs remain essentially the same for the distinct version, but with more complicated notation.

%% To avoid ambiguity, we restate the model assumptions and optimization criterion. The covariance function of the predictor $X(\cdot,\cdot)$ can be rewritten as
%% \begin{equation*}
%% C(s_1,t_1,s_2,t_2) = \expec[X(s_1,t_1)X(s_2,t_2)] = C(s_1,s_2)C(t_1,t_2).
%% \end{equation*}
%% The $\zerosnorm{\cdot}$ and $\zerotnorm{\cdot}$ norms are identical and defined as
%% \begin{equation}
%% \label{eqn:zeronorm}
%% \zeronorm{f} = \left(\intttimest f(s) C(s,t) f(t) ds dt\right)^{1/2}.
%% \end{equation}
%% The objective function \eqref{eqn:twoway-FLR} now becomes
%% \begin{eqnarray*}
%% \ell_{n \lambda}(\alpha, \beta) =
%% n^{-1} \sum_{i=1}^n\left(y_i-\int_{\T\times\T}\alpha(s) x_i(s,t) \beta(t)  dsdt\right)^2 + \lambda\|\alpha\|_0^2\|\beta\|_K^2+\lambda\|\beta\|_0^2\|\alpha\|_K^2+\lambda^2\|\alpha\|_K^2\|\beta\|_K^2.
%% \end{eqnarray*}

The eigen-structures of the kernel $K$ and the covariance function $C$, and their alignment jointly determine the performance of FLR \citep{CH06, HH07, Yuan+2010b, Cai+2012a}. Similarly, they play an important role in the theoretical property of FBLR as well. Suppose that both the reproducing kernel $K$ and the covariance function $C$ are continuous and square integrable. By Mercer's theorem, $K$ and $C$ have the
following spectral decompositions,
\begin{equation*}
  K(s,t) = \sum_{k=1}^\infty s_k^K \phi_k^K(s)\phi_k^K(t) \quad \mbox{and} \quad
  C(s,t) = \sum_{k=1}^\infty s_k^C \phi_k^C(s)\phi_k^C(t),
\end{equation*}
where $s_1^K\ge s_2^K \ge \cdots \geq 0 $ and $s_1^C\ge s_2^C \ge \cdots \ge 0 $ are the eigenvalues of $K$ and $C$ in descending order, and $\{\phi_1^K,\phi_2^K,...\}$ and $\{\phi_1^C,\phi_2^C, \ldots\}$ are the corresponding orthonormal eigenfunctions of $K$ and $C$, respectively.

The alignment of eigen-structures of $K$ and $C$ can be investigated through the idea of simultaneous diagonalization. For completeness, we provide a brief review of this idea. For more details, please see \citet{Yuan+2010b}.

Given the $\|\cdot\|_0$ and $\|\cdot\|_K$ norms for any function $f \in \H(K)$, define a new norm $\|\cdot\|_R$ that combines the two as follows,
\begin{equation*}
\|f\|_R^2 = \|f\|_0^2 + \|f\|_K^2.
\end{equation*}
Note that $\|\cdot\|_R$ is indeed a norm as discussed earlier in Section \ref{ssec:algorithm-FBLR} since $\|f\|_0^2\ne 0$ holds for any $\|f\|_K^2=0$ and $f\ne 0$. Let $R$ be the corresponding kernel associated with the $\|\cdot\|_R$ norm. Since $R$ is also continuous and square integrable, it follows from Mercer's theorem that $R$ has the following spectral decomposition,
\begin{equation*}
R(s,t) = \sum_{k=1}^\infty s_k^R \phi_k^R(s)\phi_k^R(t) ,
\end{equation*}
where $s_1^R\ge s_2^R \ge \cdots \geq 0$ and $\{\phi_1^R,\phi_2^R,...\}$ are eigenvalues and eigenfunctions of $R$ respectively.

In general, for a square integrable, symmetric, and non-negative definite function $R:\T \times \T \mapsto \R$ (similarly for $K$ and $C$), its corresponding linear operator can be defined as 
\begin{equation*}
\L_R(f)(\cdot) =\int_\T R(t,\cdot)f(t)dt.
\end{equation*}
It follows that 
\begin{equation*}
\L_R(\phi_k^R) = s_k^R\phi_k^R, ~ k=1,2,\ldots,
\end{equation*}
where $s_k^R$ and $\phi_k^R$ are the eigenvalues and eigenfunctions. 
Define the square root of the linear operator as
\begin{equation*}
\L_{R^{1/2}}(\phi_k^R) = (s_k^R)^{1/2}\phi_k^R, ~ k=1,2,\ldots .
\end{equation*}
Now consider a new linear operator $\L_T = \L_{R^{1/2}CR^{1/2}}$, that is $\L_T(f)=\L_{R^{1/2}}(\L_C(\L_{R^{1/2}}(f)))$. Since $\L_T$ is bounded linear operator, there exist eigenvalues in descending order and the corresponding eigenfunctions $\{\phi_k^T:k=1,2,\ldots\}$, such that 
\begin{equation*}
%T(s,t) = \sum_{k=1}^\infty s_k^T \phi_k^T(s)\phi_k^T(t), \mbox{ and }
\L_T(\phi_k^T) = s_k^T\phi_k^T, ~ k=1,2,\ldots.
\end{equation*}

Write $\omega_k = (s_k^{T})^{-1/2}\L_{R^{1/2}}\phi_k^T$ and
$\gamma_k = (1/s_k^T-1)^{-1}$. 
% Then it is easy to validate the following identities,
% \begin{equation}
% \label{eqn:kernelidentities}
% \langle\omega_j,\omega_k\rangle_{R} = \delta_{jk} (1/\gamma_k+1),~~
% \langle C\omega_j,\omega_k\rangle_{\L_2} = \delta_{jk},~~ \mbox{and }
% \langle \omega_j,\omega_k\rangle_{K} = \delta_{jk} /\gamma_k.
% \end{equation}
The functions $\{\omega_k:k=1,2,\ldots\}$ are essential in the proof since we will expand all of the functions of interest onto these basis functions. And the decay rate of $\gamma_k$ plays a prominent role in determining the convergence rate, understanding of which can be facilitated through the following facts. First, it is known that in the literature of nonparametric statistics, when Sobolev space is studied, $s_k^K\asymp k^{-2r} \mbox{ for some } r>1/2$ \citep{MW81}. Second, if $C$ satisfies the Sacks-Ylvisaker conditions of order $r$, then $s_k^C \asymp k^{-2(r+1)}$ \citep{SY66, SY68, SY70}. Third, if the kernel $K$ and the covariance $C$ share the same set of ordered eigenfunctions $\phi_k^K=\phi_k^C$ for all $k$, that is, perfect alignment, we have $\gamma_k =s_k^Cs_k^K$ for all $k$. Fourth, when the assumption of perfect alignment is violated, $\gamma_k\asymp s_k^Cs_k^K$ holds in many practical situations such as Sobolev space $\H$ and $C$ with Sacks-Ylvisaker condition (see Theorem 5 in \citet{Yuan+2010b}). Therefore, in what follows ,we will impose the following
conditions:\\
Condition 1: the eigenvalues of $C$ and $K$ decay as follows,
\begin{equation}
\label{eqn:decayrateassump}
s_k^C \asymp k^{-2r_c} \mbox{ for some }r_c>1/2, \mbox{ and }
s_k^K\asymp k^{-2r_k} \mbox{ for some } r_k>1/2.
\end{equation}
Condition 2: when $C$ and $K$ are simultaneously diagonalized,
\begin{equation}
  \label{eq:gamma-order}
  \gamma_k\asymp s_k^Cs_k^K\asymp k^{-2(r_c+r_k)}.
\end{equation}
Condition 3: for any functions $f, g \in \L_2(\T)$, we further assume that the
following fourth moment condition holds,
\begin{equation}
\label{eq:4th-moment-condition}
\expec \left(\int_{\T\times\T} f(s)X(s,t)g(t)dsdt \right)^4 \le M
\left( \expec \left( \int_{\T\times\T} f(s)X(s,t)g(t)dsdt \right)^2 \right)^2,
\end{equation}
for some constant $M>0$.

Note that Condition 3 is satisfied with $M=3$ when the process $X$ is assumed to be normal and is therefore weaker than the Gaussian assumption.

%--------------------------------------------------------------------
%--------------------------------------------------------------------
%--------------------------------------------------------------------
%--------------------------------------------------------------------
%--------------------------------------------------------------------

\subsection{Optimal rate of convergence}
In this section, we study the asymptotic properties of the FBLR and provide justification of the methodology proposed in Section \ref{sec:method}. We first establish a minimax upper bound for the smoothness regularization estimator in Theorem \ref{thm:upper} and then derive a minimax lower bound for all possible estimators in Theorem \ref{thm:lower}. We find that the upper bound matches the
lower bound and hence our proposed smoothness regularization estimator is rate optimal.

We assess the accuracy of the estimators by the excess prediction risk. Suppose $(X^*,Y^*)$ has the same distribution as $(X,Y)$ and is independent of the training data $\{(x_i(\cdot,\cdot),y_i), i=1,2,\ldots,n\}$. By taking expectation only with respect to $(X^*,Y^*)$, denoted by $\expecs(\cdot)$, the excess prediction risk $\calE (\halpha,\hbeta)$
is defined as follows,
\begin{eqnarray*}
  \calE (\halpha,\hbeta) &=&
  \expecs \left( Y^*-\int_{\T\times\T}\halpha(s)X^*(s,t)\hbeta(t)dsdt\right)^2
 -\expecs \left(
 Y^*-\int_{\T\times\T}\alpha_0(s)X^*(s,t)\beta_0(t)dsdt\right)^2\\
&=&\expecs \left( \int_{\T\times\T}X^*(s,t) \left( \halpha(s)\hbeta(t)-\alpha_0(s)\beta_0(t) \right)dsdt \right)^2.
%% &=&\int_{\T^4} C(s_1,s_2) C(t_1,t_2)
%% \left( \halpha(s_1)\hbeta(t_1)-\alpha_0(s_1)\beta_0(t_1) \right)
%% \left( \halpha(s_2)\hbeta(t_2)-\alpha_0(s_2)\beta_0(t_2) \right)ds_1ds_2dt_1dt_2.
\end{eqnarray*}

Theorem \ref{thm:upper} states the upper bound for the excess prediction
risk of the smoothness regularized estimator with properly chosen tuning parameter $\lambda$.
\begin{theorem}
  \label{thm:upper}
  Under Conditions 1-3, the smoothness regularization estimators $(\halpha,\hbeta)$ defined in \eqref{eqn:twowayobj} with $\lambda=O(n^{-2(r_c+r_k)/(2(r_c+r_k)+1)})$ satisfies
  \begin{equation*}
    \lim_{A\rightarrow\infty}\lim_{n\rightarrow\infty}\sup_{\substack{\alpha_0
      \in \H(K),\\ \beta_0 \in \H(K)} }
    \prob \left(\mathcal{E}(\halpha,\hbeta)\ge
    An^{-\frac{2(r_c+r_k)}{2(r_c+r_k)+1}} \right)=0.
  \end{equation*}
\end{theorem}

\noindent {\bf Remark}: By assuming the same domains, kernels, and covariance structures along the two dimensions of the two-way functional covariates, the convergence rate is determined jointly by the simultaneous diagonalization result of the covariance function $C$ and the kernel $K$ and behaves like most of the nonparametric statistical problems. Furthermore, this result demonstrates that faster decay rate of the eigenvalues of the covariance $C$ will lead to faster convergence rate of the estimator. Interestingly, this upper bound recovers the same convergence rate of the one-way FLR. We can relax these assumptions to allow different domains, kernels and/or covariance structures. The proof is essentially the same but with more complicated notation. The convergence rate will be the maximum of the convergence rates from the two domains $\max\{n^{-\frac{2(r_{c\alpha}+r_{k\alpha})}{2(r_{c\alpha}+r_{k\alpha})+1}},n^{-\frac{2(r_{c\beta}+r_{k\beta})}{2(r_{c\beta}+r_{k\beta})+1}}\}$, where the subscripts $_\alpha$ and $_\beta$ differentiate the discrepancies between the two domains corresponding to the $\alpha$ and $\beta$ dimensions, respectively.

Theorem \ref{thm:lower} provides the lower bound for the excess prediction risk over all possible estimators, which is achieved by our estimator.
\begin{theorem}
  \label{thm:lower}
  Under the same assumptions as in Theorem \ref{thm:upper}, for any estimate $(\talpha,\tbeta)$ based on the observations $\{(x_i(\cdot,\cdot),y_i): i=1,2,\ldots,n\}$, we have the following lower bound,
  \begin{equation*}
    \lim_{a\rightarrow 0}\lim_{n\rightarrow\infty}\inf_{\talpha,\tbeta}\sup_{\substack{\alpha_0 \in
      \H(K),\\ \beta_0 \in \H(K)}} \prob\left(\mathcal{E}(\talpha,\tbeta)\ge
    an^{-\frac{2(r_c+r_k)}{2(r_c+r_k)+1}}\right)=1.
  \end{equation*}
\end{theorem}

The upper bound in Theorem \ref{thm:upper} and the lower bound obtained in Theorem \ref{thm:lower} match each other. So we establish the rate optimality of our proposed smoothness regularization estimator.


==> TEX/rd_weather_v1.tex <==
%\section{Real Data: Canadian Weather}
%\label{sec:rd weather}

%We demonstrate the performance of FBLR and the existing methods on Canadian weather data. It is a classical example in functional linear regression and the aim to predict the average annual precipitation in log scale at 35 different weather stations. The traditional framework is to utilize the average daily temperature \citep[e.g.,][]{ramsay1991some,ramsay2005principal, cai2012minimax}, which is a 1D functional predictor. Since we have developed 2D functional regression and some literature have shown the relationship between temperature and precipitation in hourly data, we recollected the data of these 35 stations from \href{https://climate.weather.gc.ca/historical_data/search_historic_data_e.html}{https://climate.weather.gc.ca} and calculated the average hourly temperature for each day and base 10 logarithms of the average annual precipitation over 2002 to 2021. Therefore, the data uses 2D input of size $365 \times 24$ as the predictor to make prediction.
We demonstrate the performance of FBLR and the existing methods on Canadian weather data. We collected the data from \href{https://climate.weather.gc.ca/historical_data/search_historic_data_e.html}{the official website of the government of Canada} and calculated the hourly mean temperature for each day and log annual mean precipitation over 2002 to 2021. Therefore, the data employs 2D input of size $365 \times 24$ as the predictor to make predictions. 35 weather stations are included, all of which correspond to those mentioned in \citet{ramsay1991some,ramsay2005principal, cai2012minimax}.

We use leave-one-out method to compute the out-of-sample error. In other words, for the $i$-th stations, we use the remaining 34 stations to train the model via any methods and then make prediction for the $i$-th station. Here, as in the simulation section, we consider the following methods: FBLR, PFPCR, MFPCR, GMRF, Ridge and FLR. 
In addition, we replicate the two versions of FLR model and both use the same 1D predictor, which is generated by averaging hourly temperature for each day. 
One is FLR model in \citet{ramsay2005principal}. The other is FLR model in \citet{cai2012minimax}. To differentiate it from the FLR in simulation, we denote it as FLR\_mean. For FBLR, FLR and FLR\_mean, we employ the kernel \eqref{eq:rd-kernel}, ensuring that the slope functions fulfill periodic boundary constraints, that is, they are end-to-end joined. This kernel is also adopted in \citet{cai2012minimax}.
\be
\label{eq:rd-kernel}
    K(s,t) = 1-B_4(|s-t|)/24.
\ee

For both PFPCR and MFPCR, the maximal number of components, which achieves the lowest testing mean error, is $r^{\textrm{max}}$=5. Following the convention, we refer to them as PFPCR-$r^{\textrm{max}}$=5 and MFPCR-$r^{\textrm{max}}$=5. Again, for Ridge and FLR, we convert the two-dimensional predictor into one-dimensional through stacking columns together \carlP{Discuss about other vectorization}. BLR was not performed because the sample size is not large enough.

Figure \ref{fig:rd_weather} shows the result of leave-one-out method. 
As can be shown, while requiring more time than FLR\_mean and Ridge, FBLR is the best in terms of testing mean squared error. PFPCR and MFPCR are not much better or even worse than naive methods such as FLR and Ridge, and GMRF performs the worst. Additionally, we conduct paired t-test to compare squared error between FBLR and any other methods, and the results show that FBLR significantly outperforms all other methods at the significant level of 5\%.

\begin{figure}[!ht]
	\centerline{\includegraphics[width=.8\textwidth]{./FIGURES/rd_hourlycweather.pdf}}
	\caption{Plots of out-of-sample performance for multiple approaches in Canadian weather data, which includes the testing squared error (on the left) and computation time (on the right). The error bars are generated according to mean $\pm$ one SE.}
	\label{fig:rd_weather}
\end{figure}

Figure \ref{fig:rd_cw_betaHat} visualizes the estimated two-dimensional coefficient function $\hat\beta(\cdot,\cdot)$ in model \eqref{eqn:2dflr-other} for multiple methods for the whole data. It shows that FBLR obtains a smoother coefficient function estimation compared with the other methods. Furthermore, despite the fact that PFPCR and MFPCR are designed to produce smooth estimations, the actual estimated coefficient function is not as smooth as one might have expected, especially for the change in the day dimension. It may be due to the small sample size. \carlP{Could I remove the $\beta(.,.)$ of other six approaches to appendix}
\clearpage
\begin{figure}[!ht]
	\centerline{\includegraphics[width=.95\textwidth]{./FIGURES/rd_cw_betaHat.pdf}}
	\caption{Plots of the estimated 2D coefficient function $\hat\beta(\cdot,\cdot)$ in model \eqref{eqn:2dflr-other} by seven methods for Canadian weather data. The $x$ and $y$ axes correspond to day and hour respectively.}
	\label{fig:rd_cw_betaHat}
\end{figure}

Additionally, we examine the residuals of FBLR. The corresponding Q-Q plots are shown in figure \ref{fig:rd_cw_qqplot}, which suggests a fairly good fit of the data.

\begin{figure}[!ht]
	\centerline{\includegraphics[width=0.3\textwidth]{./FIGURES/rd_cw_QQplot.pdf}}
	\caption{Q-Q plot of the residuals. Two approaches are included, which are FBLR-$R$=2 (the left panel) and FLR\_mean (the right panel).}
	\label{fig:rd_cw_qqplot}
\end{figure}

We next want to understand the estimated slope function $\hat{\alpha}(\cdot)$ and $\hat{\beta}(\cdot)$ in FBLR corresponding to model \eqref{eqn:2dflr}. The visualizations of these two slope functions with 95\% confidence intervals are shown in figure \ref{fig:rd_cw_coef}. Some meteorological explanations for both slope functions will be provided.

The left panel shows $\hat{\alpha}(\cdot)$, which agrees with the results in the existing FLR literature \citep[e.g.,][]{ramsay2005principal, cai2012minimax}. 
The summertime confidence intervals contain zero, indicating that there is little correlation between summer temperatures and precipitation. In contrast, there is a strong peak around November and a hollow around March, which essentially computes a contrast between spring and fall. 
This pattern favors moisture-laden locations \citep{donohoe2020seasonal}. In essence, they are coastal stations close the Pacific and Atlantic oceans. They experience much warmer autumns and somewhat cooler springs than inland stations as a result of the maritime impact.

$\hat{\beta}(\cdot)$, in the right panel, reveals that more precipitation occurs in conjunction with warmer daytime and cooler nighttime. %In other words, greater precipitation accompanies greater diurnal air temperature variation. 
This pattern is in support of local breeze circulations caused by land-water temperature differences \citep[e.g.,][]{wexler1946theory,yang2006mechanisms,crosman2010sea}, which are essential to convective precipitation areas near water body (e.g. sea, gulf, lake and river). Specifically, the temperature difference between the hot landmass and the cold sea body causes onshore breezes to arise during the day. By contrast, the temperature difference reversed at night and offshore breezes predominate. %As the diurnal variation of water surface temperature is so small \citep{sverdrup1942oceans}, 
For both breezes, the major factor determining their strength is the land-water temperature difference. Therefore, the warmer daytime and the cooler nighttime produce greater land-water temperature contrasts, stronger localised diurnal breezes and corresponding stronger weather fronts over land, resulting in dense cumulus clouds and precipitation.
%This is in support of local circulations driven by temperature difference between water body (e.g. sea, gulf, lake and river) and land \citep[e.g.,][]{wexler1946theory,yang2006mechanisms,crosman2010sea}, which are crucial for convective precipitation globally \citep{crosman2010sea}. Due to greater diurnal air temperature variation, stronger weather fronts develop over land, resulting in deep cumulus clouds and precipitation.

%This is in support of the land- and sea-breeze circulation mechanisms \citep[e.g.,][]{wexler1946theory,yang2006mechanisms,crosman2010sea}, which is crucial for convective precipitation over coastal areas. Due to greater diurnal air temperature variation, stronger weather fronts develop over land, resulting in deep cumulus clouds and %occasionally
%precipitation. 

%This is in support of local circulations driven by temperature difference between water body (e.g. sea, gulf, lake and river) and land \citep[e.g.,][]{wexler1946theory,yang2006mechanisms,crosman2010sea}, which are crucial for convective precipitation globally \citep{crosman2010sea}. Due to greater diurnal air temperature variation, stronger weather fronts develop over land, resulting in deep cumulus clouds and precipitation.
%Daytime winds, i.e., sea, gulf, lake and river breezes, flow inland induced by temperature difference the hot land and cool water body. By contrast, the difference reversed at night and winds, i.e., land breezes, flow water body. For those stations with 

%This is in support of local circulations caused by land-water temperature differences \citep[e.g.,][]{wexler1946theory,yang2006mechanisms,crosman2010sea}, which contribute heavily to convective precipitation around the world\citep{crosman2010sea}. During the day, onshore winds, sometimes referred to as sea, gulf, lake, or river breezes, form as a result of the temperature differential between the hot land and the cold water surface. Conversely, the temperature difference reversed at night and offshore winds, known as land breezes, denominate. For those stations with greater diurnal temperature variation, stronger local diurnal winds induce and produce a stronger weather fronts over land, resulting in deep cumulus clouds and precipitation.


%  In coastal area, two kinds of localised winds develop in turn due to the difference in heat capacity between land and water. In the daytime, winds blow from sea toward landmass in daytime and we call them sea breezes. By contrast, winds blow from landmass toward at night and we call them land breezes. Both 
%In daytime, warmer air over land increases the strength of wind blowing from the sea and facilitates the formation of sea-breeze front. At nighttime, cooler air over land promotes the formation of land-breeze front via increasing the strength of wind blowing from the land. When powerful, both fronts create cumulus cloud and sometimes trigger precipitations.
%In daytime, warmer air over land increases the strength of wind blowing from the sea to land, while cooler air induces stronger wind blowing blowing from land to sea. When powerful, both fronts create cumulus cloud and sometimes trigger precipitations.

\begin{figure}[!ht]
	\centerline{\includegraphics[width=\textwidth]{./FIGURES/rd_cw_slope.pdf}}
	\caption{Plots of the estimated 1D coefficient functions $\hat{\alpha}(\cdot)$(the left) and $\hat{\beta}(\cdot)$(the right) in model \eqref{eqn:2dflr}. The confidence interval in dashed line is corresponding to 95\% confidence limits.}
	\label{fig:rd_cw_coef}
\end{figure}

%We can see that $\hat{\alpha}(\cdot)^{[2]}$ is negative from January to June and positive from July to December from the bottom left panel, with the seasons of spring and fall receiving greater attention. In essence, this pattern is essentially computing a contrast between spring and fall. The moisture-laden sites, where fall temperatures are higher than spring temperatures, benefit from this trend \citep{donohoe2020seasonal}, whereas stations with a strong impact from the continental climate do not. Interestingly, this pattern identified increased precipitation in stations windward side mountains at sites like Prince Rupert and Fredericton and decreased precipitation in mountains' rain shadow at stations like Kamloops, Victoria and Whitehorse.

%From the bottom right panel, $\hat{\beta}(\cdot)^{[2]}$ captures the information related to daily temperature fluctuation. With a positive relationship at midnight (2am-8am) and afternoon (1pm-6pm), more precipitation is reflected in low latitude and thus a warm condition at both the midnight and afternoon. However, for the transition period between midnight and afternoon, morning and night show the reversed relationship. Such a pattern is advantageous to the stations that warm up relatively slowly in the morning and cool down rapidly at night, which may be explained by air conditioning effects of moisture and convective precipitation brought by strong cooling.

%Additionally, we examine the residuals of FBLR-$R$=2 and FLR\_mean. The corresponding Q-Q plots are shown in figure \ref{fig:rd_cw_qqplot}. We start by examining the right panel, producing a similar finding reported in 1D FLR study \citep{ramsay2005principal, cai2012minimax}. Since 1D FLR does not account for the fact that Kamloops is located deep within the Thompson River Valley, FLR\_mean overstated the quantity of precipitation at the Kamloops station.  
%Besides, 1D FLR underestimated the precipitation at Watson station and Prince Rupert station which might be attributed to their topological positions. These two stations are located in the windward slope, where the humid sea wind hits. We next look at the Q-Q plot of FBLR-$R$=2 shown in the left panel. It indicates that FBLR-$R$=2 gives a good fit since there are no any outliers. 
%This is contributed to the second term of FBLR-$R$=2, which successfully captures the information of humidity condition. 


% I exclude these plots
\iffalse
\begin{figure}
    \centering
     \begin{subfigure}{.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./FIGURES/rd_map_flr.png}
         \caption{Prediction of FLR\_Mean}
     \end{subfigure}
     \hfill
     \begin{subfigure}{.48\textwidth}
         \includegraphics[width=\textwidth]{./FIGURES/rd_map_fblr.png}
         \caption{Prediction of FBLR-$R$=2}
     \end{subfigure}
    \hfill
    \begin{subfigure}{.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./FIGURES/rd_map_truth.png}
         \caption{Truth}
     \end{subfigure}
    \caption{Prediction of FBLR-$R$=2}
    \label{fig:three graphs}
\end{figure}
\fi


==> jmlr_coverletter_preamble.tex <==
\RequirePackage[l2tabu, orthodox]{nag}
%\documentclass{article}

% FONTS
\usepackage[T1]{fontenc}

% Import MathDesign (this brings along Bitstream Charter)
% http://www.ctan.org/tex-archive/fonts/mathdesign/
\usepackage[bitstream-charter]{mathdesign}
\usepackage{amsmath}
\usepackage[scaled=0.92]{PTSans}
\usepackage{inconsolata}

% GEOMETRY
\usepackage[
  paper  = letterpaper,
  left   = 1.5in,
  right  = 1.5in,
  top    = 1.0in,
  bottom = 1.0in,
  ]{geometry}

% COLOR
\usepackage[usenames,dvipsnames]{xcolor}
\definecolor{shadecolor}{gray}{0.9}

% SPACING and TEXT
\usepackage[final,expansion=alltext]{microtype}
\usepackage[english]{babel}
\usepackage[parfill]{parskip}

% COUNTERS
\renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
\renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
\renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

% FIGURES
\usepackage{graphicx}
\usepackage[labelfont=bf]{caption}
\usepackage[format=hang]{subcaption}

% BIBLIOGRAPHY
\usepackage{natbib}

% HYPERREF
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=Violet}
\hypersetup{linkcolor=black}
\hypersetup{urlcolor=MidnightBlue}

\newcommand{\red}[1]{\textcolor{BrickRed}{\textbf{#1}}}
\pagenumbering{gobble}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
